Extreme Star Formation

Extreme star formation includes star formation in starbursts and regions forming super star clusters. We survey the current problems in our understanding of the star formation process in starbursts and super star clusters - initial mass functions, cluster mass functions, star formation efficiencies, and radiative feedback into molecular clouds - that are critical to our understanding of the formation and survival of large star clusters, topics that will be the drivers of the observations of the next decade.

==> ExtremeSF Final Version astro-ph/ExtremeSFref.tex <==
\begin{thebibliography}{999.} %
%Overluminous HNC line emission in Arp 220, NGC 4418 and Mrk 231. Global IR 
%pumping or XDRs?
\bibitem[Aalto et al.(2007)]{2007A&A...464..193A} Aalto, S., Spaans, M., Wiedner, M.C., H\"uttemeister, S., Astron. Astrophys., \textbf{464}, 193-200 (2007) 
%Massive Star Formation in Luminous Infrared Galaxies: Giant H II Regions and Their 
%Relation to Super-Star Clusters
\bibitem[Alonso-Herrero et al.(2002)]{2002AJ....124..166A} Alonso-Herrero, 
A., Rieke, G.H., Rieke, M.J.,  Scoville, N.Z., Astron.~J., \textbf{124}, 166-182 (2002)
%Obscured Star Formation in the Central Region of the Dwarf Galaxy NGC 5253
\bibitem[Alonso-Herrero et al.(2004)]{2004ApJ...612..222A} Alonso-Herrero, A., Takagi, T., 
Baker, A.J., Rieke, G.H., 
Rieke, M.J., Imanishi, M.,  Scoville, N.Z., Astrophys.~J.,  \textbf{612}, 222-237 (2004)
%Spectra of the two brightest objects in the amorphous galaxy NGC 1569 - 
%Superluminous young star clusters-or stars in a nearby peculiar galaxy?
\bibitem[Arp and Sandage(1985)]{1985AJ.....90.1163A} Arp, H.,  Sandage, A., Astron.~J.,  
\textbf{90}, 1163-1171 (1985)
%Galaxies and their stellar populations
\bibitem[Baade(1957)]{1957Obs....77..165B} Baade, W., The Observatory,  
\textbf{77}, 165-171 (1957)
%Science with the Atacama Large Array
\bibitem[Bachiller and Cernicharo(2008)]{2008ASS...B} Bachiller, R. and Cernicharo, J., 
Science with the Atacama Large Array, (New York: Springer) (2008)
%Hubble Space Telescope Observations of Circumnuclear Star-Forming Rings in NGC 
%1097 and NGC 6951
\bibitem[Barth et al.(1995)]{1995AJ....110.1009B} Barth, A.J., Ho, L.C., Filippenko, A.V.,  Sargent, 
W.L., Astron.~J.,  \textbf{110}, 1009-1018 (1995)
\bibitem[Bastian and Goodwin(2006)]{2006MNRAS.369L...9B} Bastian, N.,  Goodwin, S.P., 
Mon. Not. R. Astron. Soc.,   \textbf{369}, L9-L13 (2006)
%Hierarchical star formation in M 51: star/cluster complexes
\bibitem[Bastian et al.(2005)]{2005A&A...443...79B} Bastian, N., Gieles, M., Efremov, Y.N.,  
Lamers, H.J.G.L.M., Astron. Astrophys.,  \textbf{443}, 79-90 (2005)
%Formation and evolutionary properties of the Galactic open cluster system
\bibitem[Battinelli and Capuzzo-Dolcetta(1991)]{1991MNRAS.249...76B} Battinelli, P.,  
Capuzzo-Dolcetta, R., Mon. Not. R. Astron. Soc.,   \textbf{249}, 76-83 (1991) 
%The Central Star Cluster of the Star-forming Dwarf Galaxy NGC 5253
\bibitem[Baumgardt et al.(2008)]{2008MNRAS.384.1231B} Baumgardt, H., Kroupa, P.,  
Parmentier, G., Mon. Not. R. Astron. Soc.,   \textbf{384}, 1231-1241 (2008) 
\bibitem[Beck et al.(1996)]{1996ApJ...457..610B} Beck, S.C., Turner, J.L., Ho, P.T.P., 
Lacy, J.H.,  Kelly, D.M., Astrophys.~J.,  \textbf{457}, 610-615 (1996)
%The Extraordinary Infrared Spectrum of NGC 1222 (Markarian 603)
\bibitem[Beck et al.(2007)]{2007AJ....134.1237B} Beck, S.C., Turner, J.L.,  Kloosterman, J., 
Astron.~J.,  \textbf{134}, 1237-1244 (2007)
%High-Resolution Radio Maps of Wolf-Rayet Galaxies: Optically Thick H II Regions?
\bibitem[Beck et al.(2000)]{2000AJ....120..244B} Beck, S.C., Turner, J.L.,  Kovo, O., 
Astron.~J.,  \textbf{120}, 244-259 (2000)
%Nonequilibrium Photodissociation Regions: Ionization-Dissociation Fronts
\bibitem[Bertoldi and Draine(1996)]{1996ApJ...458..222B} Bertoldi, F., Draine, B.T., 
Astrophys.~J.,  \textbf{458}, 222-232 (1996) 
\bibitem[Billett et al.(2002)]{2002AJ....123.1454B} Billett, O.H., Hunter, D.A., Elmegreen, B.G., 
Astron.~J.,  \textbf{123}, 1454-1475 (2002)
%The M/L* Ratio of Young Star Clusters in Galactic Mergers
\bibitem[Boily et al.(2005)]{2005ApJ...620L..27B} Boily, C.M., Lan{\c c}on, A., Deiters, S., 
Heggie, D.C., Astrophys. J.,  \textbf{620}, L27-L30 (2005)
%On the formation of massive stars
\bibitem[Bonnell et al.(1998)]{1998MNRAS.298...93B} Bonnell, I.A., Bate, M.R., 
Zinnecker, H., Mon. Not. R. Astron. Soc.,  
\textbf{298}, 93-102  (1998)
%Millimeter dust continuum emission revealing the true mass of giant molecular 
%clouds in the Small Magellanic Cloud
\bibitem[Bot et al.(2007)]{2007A&A...471..103B} Bot, C., Boulanger, F., Rubio, M., Rantakyro, F., 
Astron. Astrophys.,  \textbf{471}, 103-112 (2007)
%Intermediate to low-mass stellar content of Westerlund 1
\bibitem[Brandner et al.(2008)]{2008A&A...478..137B} Brandner, W., Clark, J.S., Stolte, A., 
Waters, R., Negueruela, I.,  Goodwin, S.P., Astron. Astrophys.,  \textbf{478}, 137-149 (2008)
\bibitem[Burbidge and Burbidge(1962)]{1962ApJ...135..694B} Burbidge, E.M., Burbidge, G.R., Astrophys.~J.,  \textbf{135}, 694-710 (1962)
%Velocity Field of M82 and its Bearing on Explosive Phenomena in that Galaxy
\bibitem[Burbidge et al.(1964)]{1964AJ.....69R.535B} Burbidge, E.M., Burbidge, G.R.,  Rubin, V.C., Astron.~J.,  \textbf{69}, 535-535 (1964)
%Star formation in NGC 5253
\bibitem[Caldwell and Phillips(1989)]{1989ApJ...338..789C} Caldwell, N.,  Phillips, M.M., Astrophys.~J., 
 \textbf{338}, 789-803 (1989)
%Dust and Recent Star Formation in the Core of NGC 5253
\bibitem[Calzetti et al.(1997)]{1997AJ....114.1834C} Calzetti, D., Meurer, G.R., Bohlin, R.C., 
Garnett, D.R., Kinney, 
A.L., Leitherer, C.,  Storchi-Bergmann, T., Astron.~J.,  \textbf{114}, 1834-1849 (1997)
%Interstellar bubbles
\bibitem[Castor et al.(1975)]{1975ApJ...200L.107C} Castor, J., McCray, R.,  Weaver, R., Astrophys. J., 
 \textbf{200}, L107-L110 (1975)
\bibitem[Chandar et al.(2003)]{2003ApJ...586..939C} Chandar, R., Leitherer, C., Tremonti, C.,  
Calzetti, D., Astrophys.~J.,  \textbf{586}, 939-958 (2003)
%NGC 3125-1: The Most Extreme Wolf-Rayet Star Cluster Known in the Local Universe
\bibitem[Chandar et al.(2004a)]{2004ApJ...604..153C} Chandar, R., Leitherer, C.,  
Tremonti, C.A.\ 2004, Astrophys.~J.,  \textbf{604}, 153-166 (2004)
%The Stellar Content of Nearby Star-forming Galaxies. III. Unravelling the Nature of the Diffuse Ultraviolet Light
\bibitem[Chandar et al.(2005)]{2005ApJ...628..210C} Chandar, R., Leitherer, 
C., Tremonti, C.A., Calzetti, D., Aloisi, A., Meurer, G.R.,  de Mello, D., Astrophys.~J., 
 \textbf{628}, 210-230 (2005)
%The Globular Cluster Systems of Five Nearby Spiral Galaxies: New Insights from 
%Hubble Space Telescope Imaging
\bibitem[Chandar et al.(2004b)]{2004ApJ...611..220C} Chandar, R., Whitmore, B.,  Lee, M.G., 
Astrophys.~J.,  \textbf{611}, 220-244 (2004)
%Wind from a starburst galaxy nucleus
\bibitem[Chevalier and Clegg(1985)]{1985Natur.317...44C} Chevalier, R.A.,  Clegg, A.W., Nature, 
 \textbf{317}, 44-45 (1985)
%Discovery of extended radio emission in the young cluster Wd1
\bibitem[Clark et al.(1998)]{1998MNRAS.299L..43C} Clark, J.S., Fender, R.P., Waters, L.B.F.M., Dougherty, S.M., Koornneef, J., Steele, I.A.,  van Blokland, A., Mon. Not. R. Astron. Soc.,  
 \textbf{299}, L43-L47 (1998)
%On the massive stellar population of the super star cluster Westerlund 1
\bibitem[Clark et al.(2005)]{2005A&A...434..949C} Clark, J.S., Negueruela, I., Crowther, P.A.,  Goodwin, 
S.P., Astron. Astrophys.,  \textbf{434}, 949-969 (2005)
%Accretion-driven core collapse and the collisional formation of massive stars
\bibitem[Clarke and Bonnell(2008)]{2008arXiv0805.1176B}Clarke, C.J.,  Bonnell, I. A., Mon. Not. R. Astron. Soc.,  in press (2008)
%
\bibitem[Condon(1992)]{1992ARA&A..30..575C} Condon, J.J., Annu. Rev. Astron. Astrophys., 
\textbf{30}, 575 (1992)
%Wolf-Rayet galaxies - an introduction and a catalog
\bibitem[Conti(1991)]{1991ApJ...377..115C} Conti, P.S.\ 1991, Astrophys.~J.,  \textbf{377}, 115-125
%Near-Infrared Observations of the Giant H II Region W49A: A Star Birth Cluster
\bibitem[Conti and Blum(2002)]{2002ApJ...564..827C} Conti, P.S.,  Blum, R.D., Astrophys.~J., 
 \textbf{564}, 827-833 (2002)
%The star cluster population of NGC 5253
\bibitem[Cresci et al.(2005)]{2005A&A...433..447C} Cresci, G., Vanzi, L.,  Sauvage, M., Astron. Astrophys.,  \textbf{433}, 447-454 (2005)
%CO in the Disk of the Barred Spiral Galaxy M83: CO (1-0), CO (2-1), and Neutral Gas
\bibitem[Crosthwaite et al.(2002)]{2002AJ....123.1892C} Crosthwaite, L.P., Turner, J.L., 
Buchholz, L., Ho, P.T.P., and Martin, R.N., Astron.~J.,  \textbf{123}, 1892-1912 (2002)
%CO(1-0), CO(2-1), and Neutral Gas in NGC 6946: Molecular Gas in a Late-Type, Gas-Rich, Spiral Galaxy
\bibitem[Crosthwaite and Turner(2007)]{2007AJ....134.1827C} Crosthwaite, L.P.,  Turner, J.L., 
Astron.~J.,  \textbf{134}, 1827-1842 (2007)
%Properties of hot stars in the Wolf-Rayet galaxy NGC 5253 from ISO-SWS spectroscopy
\bibitem[Crowther et al.(1999)]{1999MNRAS.304..654C} Crowther, P.A., Beck, S.C., Willis, A.J., 
Conti, P.S., Morris, P.W., and Sutherland, R.S., Mon. Not. R. Astron. Soc.,   \textbf{304}, 654-668 (1999)
%A census of the Wolf-Rayet content in Westerlund 1 from near-infrared imaging and 
%spectroscopy
\bibitem[Crowther et al.(2006)]{2006MNRAS.372.1407C} Crowther, P.A., 
Hadfield, L.J., Clark, J.S., Negueruela, I.,  Vacca, W.D., Mon. Not. R. Astron. Soc.,  
 \textbf{372}, 1407-1424 (2006)
%Molecular gas in the Galactic center region. II. Gas mass and N_, = H_2/I_^(12)CO 
%conversion based on a C^(18)O(J = 1 -> 0) survey
\bibitem[Dahmen et al.(1998)]{1998A&A...331..959D} Dahmen, G., Huttemeister, S., Wilson, T.L.,  Mauersberger, R.\ 1998, Astron. Astrophys.,  \textbf{331}, 959-976 
%Mid-Infrared Spectral Diagnostics of Nuclear and Extranuclear Regions in Nearby 
%Galaxies
\bibitem[Dale et al.(2006)]{2006ApJ...646..161D} Dale, D.A., et al., Astrophys.~J., 
\textbf{646}, 161-173 (2006)
%The Milky Way in Molecular Clouds: A New Complete CO Survey
\bibitem[Dame et al.(2001)]{2001ApJ...547..792D} Dame, T.M., Hartmann, D.,  Thaddeus, P.\ 2001, Astrophys.~J., \textbf{547}, 792-813
%On the Distance and Molecular Environment of Westerlund 2 and HESS J1023-575
%\bibitem[Dame 2007]{2007ApJ...665L.163D} Dame, T.M., Astrophys. J.,  \textbf{665},   L163-L166 (2007)
\bibitem[de Grijs(2007)]{2007arXiv0711.3540D} 
de Grijs, R. to appear in "Young massive star clusters---Initial conditions and environments", 
E. Perez, R. de Grijs, R. M. Gonzalez Delgado, eds., (Springer: Dordrecht)
e-prints, 711, arXiv:0711.3540 (2007)
%Star cluster formation and evolution in nearby starburst galaxies - II. Initial conditions
\bibitem[de Grijs et al.(2003)]{2003MNRAS.343.1285D} de Grijs, R., ers, P., Bastian, N., Lynds, R., 
Lamers, H.J.G.L.M.,  O'Neil, E.J., Mon. Not. R. Astron. Soc.,   \textbf{343}, 1285-1300 (2003)
%IRAS observations of Shapley-Ames galaxies
\bibitem[de Jong et al.(1984)]{1984ApJ...278L..67D} de Jong, T., Clegg, P.E., 
Rowan-Robinson, M., Soifer, B.T., Habing,
H.J., Houck, J.R., Aumann, H.H.,  Raimond, E., Astrophys. J.,  \textbf{278}, L67-L70 (1984)
%The Population of Massive Stars in R136 from Faint Object Camera Ultraviolet Observations
\bibitem[de Marchi et al.(1993)]{1993ApJ...419..658D} de Marchi, G., Nota, 
A., Leitherer, C., Ragazzoni, R.,  Barbieri, C., Astrophys.~J.,  \textbf{419}, 658-669 (1993)
%The Structure of the Super--Star Clusters in NGC 1569 from HST WFPC2 Images
\bibitem[de Marchi et al.(1997)]{1997ApJ...479L..27D} de Marchi, G., 
Clampin, M., Greggio, L., Leitherer, C., Nota, A.,  Tosi, M.,  Astrophys. J.,  
\textbf{479}, L27-L30 (1997)
%NGC 3576 and NGC 3603: Two Luminous Southern H II Regions Observed at High Resolution with the Australia Telescope Compact Array
\bibitem[de Pree et al.(1999)]{1999AJ....117.2902D} de Pree, C.G., Nysewander, M.C.,  Goss, W.M., Astron.~J.,  
\textbf{117}, 2902-2918 (1999)
%Ultracompact H II regions: are their lifetimes extended by dense, warm environments?
\bibitem[de Pree et al.(1995)]{1995RMxAA..31...39D} de Pree, C.G., Rodriguez, L.F., 
and Goss, W.M., Revista Mexicana de Astronomia y Astrofisica,  \textbf{31}, 39-44 (1995)
%Carbon monoxide as an extragalactic mass tracer
\bibitem[Dickman et al.(1986)]{1986ApJ...309..326D} Dickman, R.L., Snell, R.L.,  
Schloerb, F.P., Astrophys.~J.,  \textbf{309}, 326-330 (1986)
%Modeling the Pan-Spectral Energy Distribution of Starburst Galaxies. I. The Role of ISM 
%Pressure and the Molecular Cloud Dissipation Timescale
\bibitem[Dopita et al.(2005)]{2005ApJ...619..755D} Dopita, M.A., et al., Astrophys.~J.,  
\textbf{619}, 755-778 (2005) 
%Modeling the Pan-Spectral Energy Distribution of Starburst Galaxies. II. Control of the 
%H II Region Parameters
%\bibitem[Dopita et al.\ 2006a]
%{2006ApJ...647..244D} Dopita, M.A., et al., Astrophys.~J., 647, 244-255 (2006)
%Modeling the Pan-Spectral Energy Distribution of Starburst Galaxies. III. Emission Line Diagnostics of Ensembles of Evolving H II Regions
\bibitem[Dopita et al.(2006)]{2006ApJS..167..177D} Dopita, M.A., et al., ApJS,  \textbf{167}, 
177-200 (2006)
%Far-Infrared Polarization by Absorption in the Molecular Cloud Sagittarius B2
\bibitem[Dowell(1997)]{1997ApJ...487..237D} Dowell, C.D., Astrophys.~J.,  \textbf{487}, 237-247 (1997)
%Rotating Nuclear Rings and Extreme Starbursts in Ultraluminous Galaxies
\bibitem[Downes and Solomon(1998)]{1998ApJ...507..615D} Downes, D.,  Solomon, P.M., 
Astrophys.~J.,  \textbf{507}, 615-654 (1998)
%Molecular gas mass and far-infrared emission from distant luminous galaxies
\bibitem[Downes et al.(1993)]{1993ApJ...414L..13D} Downes, D., Solomon, P.M.,  
Radford, S.J.E., Astrophys. J.,  \textbf{414}, L13-L16 (1993)
%Structure of Stationary Photodissociation Fronts
\bibitem[Draine and Bertoldi(1996)]{1996ApJ...468..269D} Draine, B.T.,  Bertoldi, F., 
Astrophys.~J.,  \textbf{468}, 269-289 (1996)
%Ultracompact structure in the H II region W49N
\bibitem[Dreher et al.(1984)]{1984ApJ...283..632D} Dreher, J.W., Johnston, K.J., 
Welch, W.J.,  Walker, R.C., Astrophys.~J.,  \textbf{283}, 632-639 (1984)
%The Dense Galactic Starburst NGC 3603. I. HST/FOS Spectroscopy of Individual Stars 
%in the Core and the source of Ionization and Kinetic Energy
\bibitem[Drissen et al.(1995)]{1995AJ....110.2235D} Drissen, L., Moffat, A.F.J., Walborn, N.R.,  Shara, M.M., Astron.~J.,  \textbf{110}, 2235-2241 (1995)
%Stellar Content of the Galactic Starburst Template NGC 3603 from Adaptive Optics 
%Observations
\bibitem[Eisenhauer et al.(1998)]{1998ApJ...498..278E} Eisenhauer, F., Quirrenbach, A., 
Zinnecker, H.,  Genzel, R., Astrophys.~J.,  \textbf{498}, 278-292 (1998)
%On the Rapid Collapse and Evolution of Molecular Clouds
\bibitem[Elmegreen(2007)]{2007ApJ...668.1064E} Elmegreen, B.G., Astrophys.~J.,  
\textbf{668}, 1064-1082 (2007)
%The Stellar Initial Mass Function in 2007: A Year for Discovering Variations
\bibitem[Elmegreen(2008)]{2008arXiv0803.3154E} Elmegreen, B.G., ArXiv e-prints, 803, 
arXiv:0803.3154 (2008)
%Sequential formation of subgroups in OB associations
%\bibitem[Elmegreen and Lada 1977]{1977ApJ...214..725E} Elmegreen, B.G.,  Lada, C.J., 
%Astrophys.~J.,  \textbf{214}, 725-741 (1977)
%Survival and disruption of galactic substructure
\bibitem[Fall and Rees(1977)]{1977MNRAS.181P..37F} Fall, S.M.,  Rees, M.J., 
Mon. Not. R. Astron. Soc.,   \textbf{181}, 37P-42P (1977)
%Dynamical Evolution of the Mass Function of Globular Star Clusters
\bibitem[Fall and Zhang(2001)]{2001ApJ...561..751F} Fall, S.M.,  Zhang, Q., 
Astrophys.~J.,  \textbf{561}, 751-765 (2001)
%The Age Distribution of Massive Star Clusters in the Antennae Galaxies
\bibitem[Fall et al.(2005)]{2005ApJ...631L.133F} Fall, S.M., Chandar, R.,  Whitmore, B.C., Astrophys. J.,  \textbf{631}, L133-L136 (2005)
%Massive Stars and The Creation of our Galactic Center
\bibitem[Figer(2003)]{2003ANS...324..255F} Figer, D.F., Astronomische Nachrichten Supplement, 
 \textbf{324}, 255-261 (2003)
%Young Massive Clusters in the Galactic Center
\bibitem[Figer(2004)]{2004ASPC..322...49F} Figer, D.F., The Formation and Evolution of Massive Young 
Star Clusters,  \textbf{322}, 49 (2004)
%An upper limit to the masses of stars
\bibitem[Figer(2005)]{2005Natur.434..192F} Figer, D.F., Nature,  \textbf{434}, 192-194 (2005)
%Massive Star Formation in the Galactic Center
\bibitem[Figer(2008)]{2008arXiv0803.1619F} Figer, D.F., ArXiv e-prints, 803, arXiv:0803.1619 (2008)
%Young Massive Clusters
%\bibitem[Figer(2008)]{2008arXiv0801.4178F} Figer, D.F., ArXiv e-prints, 801, arXiv:0801.4178 (2008)
\bibitem[Figer(2008)]{2008IAUS..250..247F} Figer, D.F., in Massive Stars as Cosmic
Engines, IAU Symposium, \textbf{250}, 247-256 (2008)
%Hubble Space Telescope/NICMOS Observations of Massive Stellar Clusters near the 
%Galactic Center
\bibitem[Figer et al.(1999)]{1999ApJ...525..750F} Figer, D.F., Kim, S.S., Morris, M., Serabyn, E., 
Rich, R.M., and McLean, I.S., Astrophys.~J.,  \textbf{525}, 750-758 (1999)
%The Pistol Star
\bibitem[Figer et al.(1998)]{1998ApJ...506..384F} Figer, D.F., Najarro, F., Morris, M., McLean, I.S., Geballe, T.R., Ghez, A.M.,  Langer, N., Astrophys.~J.,  \textbf{506}, 384-404 (1998)
%Near-Infrared Integral Field Spectroscopy and Mid-Infrared Spectroscopy of the 
%Starburst Galaxy M82
\bibitem[F\"orster Schreiber et al.(2001)]{2001ApJ...552..544F} F\"orster Schreiber, N.M., 
Genzel, R., Lutz, D., Kunze, D.,  Sternberg, A., Astrophys.~J.,  \textbf{552}, 544-571 (2001)
%Variations of the Mid-IR Aromatic Features inside and among Galaxies
\bibitem[Galliano et al.(2008)]{2008ApJ...679..310G} Galliano, F., Madden, S.C., Tielens, 
A.G.G.M., Peeters, E., and Jones, A.P., Astrophys.~J.,  \textbf{679}, 310-345 (2008)
%The Star Formation Rate and Dense Molecular Gas in Galaxies
\bibitem[Gao and Solomon(2004)]{2004ApJ...606..271G} Gao, Y.,  Solomon, P.M., 
Astrophys.~J.,  \textbf{606}, 271-290 (2004)
%Colors and Magnitudes of Some Star Clusters in the Magellanic Clouds
\bibitem[Gascoigne and Kron(1952)]{1952PASP...64..196G} Gascoigne, S.C.B.,  
Kron, G.E., Publ. Astron. Soc. Pac.,   \textbf{64}, 196-200 (1952)
%The Sagittarius B2 Star-forming Region. I. Sensitive 1.3 Centimeter Continuum 
%Observations
\bibitem[Gaume et al.(1995)]{1995ApJ...449..663G} Gaume, R.A., Claussen, M.J., 
de Pree, C.G., Goss, W.M.,  Mehringer, D.M., Astrophys.~J.,  \textbf{449}, 663-673  (1995)
%Star bursts and the extraordinary galaxy NGC 3690
\bibitem[Gehrz et al.(1983)]{1983ApJ...267..551G} Gehrz, R.D., Sramek, R.A.,  
Weedman, D.W., Astrophys.~J.,  \textbf{267}, 551-562 (1983)
%A Search for Old Star Clusters in the Large Magellanic Cloud
%\bibitem[Geisler et al.\ 1997]{1997AJ....114.1920G} Geisler, D., Bica, E., Dottori, H., 
%Claria, J.J., Piatti, A.E., and Santos, J.F.C., Jr., Astron.~J.,  \textbf{114}, 1920-1932 (1997)
%Extragalactic Results from the Infrared Space Observatory
\bibitem[Genzel and Cesarsky(2000)]{2000ARA&A..38..761G} Genzel, R.,  
Cesarsky, C.J.\ 2000, Annu. Rev. Astron. Astrophys., \textbf{38}, 761-814
%What Powers Ultraluminous IRAS Galaxies?
\bibitem[Genzel et al.(1998)]{1998ApJ...498..579G} Genzel, R., et al.,  Astrophys.~J.,  
\textbf{498}, 579-605 (1998)
%The Galactic Center HE I Stars: Remains of a Dissolved Young Cluster?
%\bibitem[Gerhard 2001]{2001ApJ...546L..39G} Gerhard, O., Astrophys. J.,  \textbf{546}, L39-L42  (2001)
%An alternative method to study star cluster disruption
\bibitem[Gieles and Bastian(2008)]{2008A&A...482..165G} Gieles, M.,  Bastian, N., 
Astron. Astrophys.,  \textbf{482}, 165-171 (2008)
%The GALEX Ultraviolet Atlas of Nearby Galaxies
\bibitem[Gil de Paz et al.(2007)]{2007ApJS..173..185G} Gil de Paz, A., et al., ApJS, 
 \textbf{173}, 185-255 (2007)
%nfrared spectroscopy of massive stellar clusters in starbursts
\bibitem[Gilbert(2002)]{2002PhDT........15G} Gilbert, A.M., Ph.D.Dissertation, 
University of California, Berkeley (2002)
%Infrared Spectroscopy of a Massive Obscured Star Cluster in the Antennae Galaxies 
%(NGC 4038/9) with NIRSPEC
\bibitem[Gilbert et al.(2000)]{2000ApJ...533L..57G} Gilbert, A.M., et al., Astrophys. J.,  
\textbf{533}, L57-L60 (2000)
%The initial conditions of young globular clusters in the Large Magellanic Cloud
\bibitem[Goodwin(1997)]{1997MNRAS.286..669G} Goodwin, S.P.\ 1997, Mon. Not. R. 
Astron. Soc.,   \textbf{286}, 669-680 (1997) 
%WFPC2 Imaging of the Starburst Galaxy NGC 5253
\bibitem[Gorjian(1996)]{1996AJ....112.1886G} Gorjian, V., Astron.~J.,  \textbf{112}, 1886-1893 (1996)
%Infrared Emission from the Radio Supernebula in NGC 5253: A Proto-Globular Cluster?
\bibitem[Gorjian et al.(2001)]{2001ApJ...554L..29G} Gorjian, V., Turner, J.L.,  Beck, S.C., 
Astrophys. J.,  \textbf{554}, L29-L33 (2001)
%Destruction of the Galactic Globular Cluster System
\bibitem[Gnedin and Ostriker(1997)]{1997ApJ...474..223G} Gnedin, O.Y.,  Ostriker, J.P., 
Astrophys.~J.,  \textbf{474}, 223-255 (1997)
%A Morphological Diagnostic for Dynamical Evolution of Wolf-Rayet Bubbles
\bibitem[Gruendl et al.(2000)]{2000AJ....120.2670G} Gruendl, R.A., Chu, Y.-H., Dunne, B.C.,  
Points, S.D., Astron.~J.,  \textbf{120}, 2670-2678 (2000)
%Exceptional H2 emission in the Antennae galaxies: Pre-starburst shocks from the galaxy collision
\bibitem[Haas et al.(2005)]{2005A&A...433L..17H} Haas, M., Chini, R.,  Klaas, U., Astron. 
Astrophys.,  \textbf{433}, L17-L20 (2005)
%How extreme are the Wolf-Rayet clusters in NGC3125?*
\bibitem[Hadfield and Crowther(2006)]{2006MNRAS.368.1822H} Hadfield, L.J.,  Crowther, P.A., 
Mon. Not. R. Astron. Soc.,   \textbf{368}, 1822-1832 (2006)
%The Initial Mass Function of the Massive Star-forming Region NGC 3603 from Near-
%Infrared Adaptive Optics Observations
\bibitem[Harayama et al.(2008)]{2008ApJ...675.1319H} Harayama, Y., Eisenhauer, F.,  
Martins, F., Astrophys.~J.,  \textbf{675}, 1319-1342 (2008)
%Cluster Mass and Metallicity Distributions: Reconstructing the Events During Halo Formation
\bibitem[Harris(2002)]{2002IAUS..207..545H} Harris, W.E., Extragalactic Star Clusters, 
 \textbf{207}, 545  (2002)
%A Catalog of Parameters for Globular Clusters in the Milky Way
\bibitem[Harris(1996)]{1996AJ....112.1487H} Harris, W.E., Astron.~J.,  \textbf{112}, 1487-1488 (1996)
%Issues in the Formation of Globular Cluster Systems
\bibitem[Harris(1998)]{1998ASPC..136...33H} Harris, W.E., in Galactic Halos, ed. D. Zaritsky,
(San Francisco:A. S. P.)  \textbf{136}, 33-41 (1998)
%Star Clusters in Astrophysical Quantities.
\bibitem[Harris and Harris(2000)]{2000Harrissquare} Harris, W.E.,  Harris, H.C., in
 Astrophysical Quantities, ed. A. N. Cox (Springer, London), 545-568 (2000)
%Supergiant molecular clouds and the formation of globular cluster systems
\bibitem[Harris and Pudritz(1994)]{1994ApJ...429..177H} Harris, W.E.,  Pudritz, R.E., 
Astrophys.~J.,  \textbf{429}, 177-191 (1994)
%The Mid-Infrared Spectra of Normal Galaxies
\bibitem[Helou et al.(2000)]{2000ApJ...532L..21H} Helou, G., Lu, N.Y., 
Werner, M.W., Malhotra, S.,  Silbermann, N., Astrophys. J.,  \textbf{532}, L21-L24 (2000)
%A Spitzer Space Telescope Infrared Spectrograph Survey of Warm Molecular 
%Hydrogen in Ultraluminous Infrared Galaxies
\bibitem[Higdon et al.(2006)]{2006ApJ...648..323H} Higdon, S.J.U., Armus, 
L., Higdon, J.L., Soifer, B.T.,  Spoon, H.W.W., Astrophys.~J.,  \textbf{648}, 323-339 (2006)
%The effect of mass loss on the dynamical evolution of a stellar system - Analytic approximations
\bibitem[Hills(1980)]{1980ApJ...235..986H} Hills, J.G., Astrophys.~J.,  \textbf{235}, 986-991 (1980)
%Brackett line spectroscopy of bursts of star formation in the nuclei of galaxies
\bibitem[Ho et al.(1990)]{1990ApJ...349...57H} Ho, P.T.P., Beck, S.C.,  Turner, J.L., Astrophys.~J., 
 \textbf{349}, 57-66 (1990)
%Dynamical Evidence for Massive, Young Globular Clusters in NGC 1569
\bibitem[Ho and Filippenko(1996)]{1996ApJ...466L..83H} Ho, L.C.,  Filippenko, A.V., Astrophys. J., 
 \textbf{466}, L83-L86 (1996a)
%High-Dispersion Spectroscopy of a Luminous, Young Star Cluster in NGC 1705: Further Evidence for Present-Day Formation of Globular Clusters
\bibitem[Ho and Filippenko(1996)]{1996ApJ...472..600H} Ho, L.C.,  Filippenko, A.V., 
Astrophys.~J.,  \textbf{472}, 600-610  (1996b)
%Studies of the Large Magellanic Cloud. V. The Young Populous Clusters
\bibitem[Hodge(1961)]{1961ApJ...133..413H} Hodge, P.W., Astrophys.~J.,  \textbf{133}, 413-419 (1961)
%Photodissociation regions in the interstellar medium of galaxies
\bibitem[Hollenbach and Tielens(1999)]{1999RvMP...71..173H} Hollenbach, D.J.,  Tielens, A.G.G.M., Reviews of Modern Physics,  \textbf{71}, 173-230 (1999)
%Planetary Camera observations of NGC 1275 - Discovery of a central population of 
%compact massive blue star clusters
\bibitem[Holtzman et al.(1992)]{1992AJ....103..691H} Holtzman, J.A., et al., Astron.~J., 
 \textbf{103}, 691-702 (1992)
%Massive star formation in the W49 giant molecular cloud: Implications for the formation 
%of massive star clusters
\bibitem[Homeier and Alves(2005)]{2005A&A...430..481H} Homeier, N.L.,  Alves, J., Astron. 
Astrophys.,  \textbf{430}, 481-489 (2005)
%Nucleosynthesis and Mixing in Cassiopeia A
\bibitem[Hughes et al.(2000)]{2000ApJ...528L.109H} Hughes, J.P., Rakowski, C.E., Burrows, 
D.N.,  Slane, P.O., Astrophys. J.,  \textbf{528}, L109-L113 (2000)
%The Intermediate Stellar Mass Population in R136 Determined from Hubble Space 
%Telescope Planetary Camera 2 Images
\bibitem[Hunter et al.(1995)]{1995ApJ...448..179H} Hunter, D.A., Shaya, 
E.J., Holtzman, J.A., Light, R.M., O'Neil, E.J., Jr.,  Lynds, R., Astrophys.~J.,  \textbf{448}, 179-194 (1995)
%The Intermediate-Mass Population in the Core of the R136 Star Cluster
\bibitem[Hunter et al.(1996)]{1996ApJ...459L..27H} Hunter, D.A., O'Neil, E.J., Jr., Lynds, R., 
Shaya, E.J., Groth, E.J., and Holtzman, J.A., Astrophys. J.,  \textbf{459}, L27-L30 (1996)
%The Star Clusters in the Starburst Irregular Galaxy NGC 1569
\bibitem[Hunter et al.(2000)]{2000AJ....120.2383H} Hunter, D.A., 
O'Connell, R.W., Gallagher, J.S.,  Smecker-Hane, T.A., Astron.~J.,  \textbf{120}, 
2383-2401 (2000)
%Carbon monoxide in the Magellanic Clouds
\bibitem[Israel et al.(1986)]{1986ApJ...303..186I} Israel, F.P., de Graauw, T., van de Stadt, H.,  
de Vries, C.P., Astrophys.~J.,  \textbf{303}, 186-197 (1986)
%The Spectral Energy Distributions of Infant Super-Star Clusters in Henize 2-10 from 7 
%Millimeters to 6 Centimeters
\bibitem[Johnson and Kobulnicky(2003)]{2003ApJ...597..923J} Johnson, K.E.,  
Kobulnicky, H.A., Astrophys.~J.,  \textbf{597}, 923-928 (2003)
%
\bibitem[Johnson et al.(2003)]{2003AJ....126..101J} Johnson, K.E., Indebetouw, R.,  
Pisano, D.J., Astron.~J.,  \textbf{126}, 101-112 (2003)
%The Hubble Flow around the Centaurus A/M83 Galaxy Complex
\bibitem[Karachentsev et al.(2007)]{2007AJ....133..504K} Karachentsev, I.D., et al.\ 2007, 
Astron.~J.,  \textbf{133}, 504-517 (2007)
%[Si II], [Fe II], [C II], and H2 Emission from Massive Star-forming Regions
\bibitem[Kaufman et al.(2006)]{2006ApJ...644..283K} Kaufman, M.J., 
Wolfire, M.G.,  Hollenbach, D.J., Astrophys.~J.,  \textbf{644}, 283-299 (2006)
%Far-Infrared and Submillimeter Emission from Galactic and Extragalactic 
%Photodissociation Regions
\bibitem[Kaufman et al.(1999)]{1999ApJ...527..795K} Kaufman, M.J., 
Wolfire, M.G., Hollenbach, D.J.,  Luhman, M.L., Astrophys.~J.,  \textbf{527}, 795-813 (1999)
%Brackett alpha and gamma Observations of Starburst and Seyfert Galaxies
\bibitem[Kawara et al.(1989)]{1989ApJ...337..230K} Kawara, K., Nishida, M.,  Phillips, M.M., 
Astrophys.~J.,  \textbf{337}, 230-235 (1989)
%Structural properties of giant H II regions in nearby galaxies
\bibitem[Kennicutt(1984)]{1984ApJ...287..116K} Kennicutt, R.C., Jr., Astrophys.~J.,  
\textbf{287}, 116-130 (1984)
%Star Formation in Galaxies Along the Hubble Sequence
\bibitem[Kennicutt(1998)]{1998ARAA..36..189K} Kennicutt, R.C., Jr., Annu. Rev. 
Astron. Astrophys.,  \textbf{36}, 189-232 (1998)
%The Global Schmidt Law in Star-forming Galaxies
\bibitem[Kennicutt(1998b)]{1998ApJ...498..541K} Kennicutt, R.C., Jr., Astrophys.~J.,  
\textbf{498}, 541-552 (1998)
%SINGS: The SIRTF Nearby Galaxies Survey
%\bibitem[Kennicutt et al.\ 2003]{2003PASP..115..928K} Kennicutt, R.C., Jr., et al., 
%Publ. Astron. Soc. Pac.,   \textbf{115}, 928-952 (2003)
%N-Body Simulations of Compact Young Clusters near the Galactic Center
\bibitem[Kim et al.(2000)]{2000ApJ...545..301K} Kim, S.S., Figer, D.F., 
Lee, H.M.,  Morris, M., Astrophys.~J.,  \textbf{545}, 301-308 (2000)
%The Arches Cluster Mass Function
\bibitem[Kim et al.(2007)]{2007JKAS...40..153K} Kim, S.S., Figer, D.F., Kudritzki, R.P., 
and Najarro, F., Journal of Korean Astronomical Society,  \textbf{40}, 153-155 (2007)
%Dynamical Friction on Galactic Center Star Clusters with an Intermediate-Mass Black 
%Hole
\bibitem[Kim et al.(2004)]{2004ApJ...607L.123K} Kim, S.S., Figer, D.F.,  Morris, M., Astrophys. J., 
 \textbf{607}, L123-L126 (2004)
%Signatures of the Youngest Starbursts: Optically Thick Thermal Bremsstrahlung Radio 
%Sources in Henize 2-10
\bibitem[Kobulnicky and Johnson(1999)]{1999ApJ...527..154K} Kobulnicky, H.A.,  
Johnson, K.E., Astrophys.~J.,  \textbf{527}, 154-166 (1999)
%Inflows and Outflows in the Dwarf Starburst Galaxy NGC 5253: High-Resolution H i Observations
\bibitem[Kobulnicky and Skillman(2008)]{2008AJ....135..527K} Kobulnicky, H.A.,  
Skillman, E.D., Astron.~J.,  \textbf{135}, 527-537 (2008)
%On the upper limit on stellar masses in the Large Magellanic Cloud cluster R136
\bibitem[Koen(2006)]{2006MNRAS.365..590K} Koen, C., Mon. Not. R. Astron. Soc.,   
\textbf{365}, 590-594 (2006)
%On the variation of the initial mass function
\bibitem[Kroupa(2001)]{2001MNRAS.322..231K} Kroupa, P., Mon. Not. R. Astron. Soc.,  
 \textbf{322}, 231-246 (2001)
 %On the mass function of star clusters
\bibitem[Kroupa and Boily(2002)]{2002MNRAS.336.1188K} Kroupa, P.,  
Boily, C.M., Mon. Not. R. Astron. Soc.,  \textbf{336}, 1188-1194 (2002)
\bibitem[Krumholz et al.(2006)]{2006ApJ...653..361K} Krumholz, M.R., Matzner, C.D.,  
McKee, C.F., Astrophys.~J.,  \textbf{653}, 361-382 (2006)
\bibitem[Krumholz and Tan(2007)]{2007ApJ...654..304K} Krumholz, M.R.,  Tan, J.C., 
Astrophys.~J.,  \textbf{654}, 304-315 (2007)
\bibitem[Lada et al.(1984)]{1984ApJ...285..141L} Lada, C.J., Margulis, M.,  Dearborn, D., 
Astrophys.~J.,  \textbf{285}, 141-152 (1984)
\bibitem[Lada and Lada(2003)]{2003ARA&A..41...57L} Lada, C.J.,  Lada, E.A., Annu. 
Rev. Astron. Astrophys.,  \textbf{41}, 57-115 (2003)
%A VLA H92? Recombination Line Study of the Arched Filament H II Complex Near the Galactic Center
\bibitem[Lang et al.(2001)]{2001AJ....121.2681L} Lang, C.C., Goss, W.M.,  Morris, M., Astron.~J., 
 \textbf{121}, 2681-2705 (2001)
%Anatomy of a young massive star cluster: NGC 1569-B
\bibitem[Larsen et al.(2008)]{2008MNRAS.383..263L} Larsen, S.S., Origlia, 
L., Brodie, J.,  Gallagher, J.S., Mon. Not. R. Astron. Soc.,   \textbf{383}, 263-276 (2008)
%Starburst99: Synthesis Models for Galaxies with Active Star Formation
\bibitem[Leitherer et al.(1999)]{1999ApJS..123....3L} Leitherer, C., et al., ApJS,  \textbf{123}, 3-40 (1999)
%X-ray-induced chemistry of interstellar clouds.
\bibitem[Lepp and Dalgarno(1996)]{1996A&A...306L..21L} Lepp, S.,  Dalgarno, A., Astron. 
Astrophys.,  \textbf{306}, L21-L24 (2006)
%SWIRE: The SIRTF Wide-Area Infrared Extragalactic Survey
\bibitem[Lonsdale et al.(2003)]{2003PASP..115..897L} Lonsdale, C.J., et al., Publ. Astron. 
Soc. Pac.,   \textbf{115}, 897-927 (2003)
%Faint [O iv] emission from starburst galaxies
\bibitem[Lutz et al.(1998)]{1998A&A...333L..75L} Lutz, D., Kunze, D., Spoon, H.W.W.,  Thornley, M.D., Astron. Astrophys.,  \textbf{333}, L75-L78 (1998)
%Evidence for an Explosion in the Center of the Galaxy M82.
\bibitem[Lynds and Sandage(1963)]{1963AJ.....68R.284L} Lynds, C.R.,  Sandage, A.R., 
Astron.~J.,  \textbf{68}, 285 (1963)
%Surface brightness profiles and structural parameters for 53 rich stellar clusters in the Large Magellanic Cloud
\bibitem[Mackey and Gilmore(2003)]{2003MNRAS.338...85M} Mackey, A.D.,  Gilmore, 
G.F., Mon. Not. R. Astron. Soc.,   \textbf{338}, 85-119 (2003)
%I(CO)/N(H2) conversions and molecular gas abundances in spiral and irregular galaxies
\bibitem[Maloney and Black(1988)]{1988ApJ...325..389M} Maloney, P.,  Black, J.H., 
Astrophys.~J.,  \textbf{325}, 389-401 (1988)
%X-Ray--irradiated Molecular Gas. I. Physical Processes and General Results
\bibitem[Maloney et al.(1996)]{1996ApJ...466..561M} Maloney, P.R., 
Hollenbach, D.J.,  Tielens, A.G.G.M., Astrophys.~J.,  \textbf{466}, 561-584 (1996) 
%Formaldehyde Densitometry of Starburst Galaxies
\bibitem[Mangum et al.(2008)]{2008ApJ...673..832M} Mangum, J.G., Darling, 
J., Menten, K.M.,  Henkel, C., Astrophys.~J.,  \textbf{673}, 832-846 (2008)
%An Ultraviolet through Infrared Look at Star Formation and Super Star Clusters in Two Circumnuclear Starburst Rings
\bibitem[Maoz et al.(2001)]{2001AJ....121.3048M} Maoz, D., Barth, A.J., 
Ho, L.C., Sternberg, A.,  Filippenko, A.V., Astron.~J.,  \textbf{121}, 3048-3074 (2001)
%Hubble Space Telescope Ultraviolet Images of Five Circumnuclear Star-Forming Rings
\bibitem[Maoz et al.(1996)]{1996AJ....111.2248M} Maoz, D., Barth, A.J., 
Sternberg, A., Filippenko, A.V., Ho, L.C., Macchetto, F.D., Rix, H.-W., 
and Schneider, D.P., Astron.~J.,  \textbf{111}, 2248-2264 (1996)
%An Atlas of Hubble Space Telescope Ultraviolet Images of Nearby Galaxies
\bibitem[Maoz et al.(1996)]{1996ApJS..107..215M} Maoz, D., Filippenko, A.V., Ho, L.C., Macchetto, F.D., 
Rix, H.-W.,  Schneider, D.P., ApJS,  \textbf{107}, 215-226 (1996)
%Methanol detection in M 82
\bibitem[Mart\'in et al.(2006)]{2006A&A...450L..13M} Mart\'in, S., Mart\'in-Pintado, J.,  
Mauersberger, R., Astron. Astrophys.,  \textbf{450}, L13-L16 (2006)
%A 2 Millimeter Spectral Line Survey of the Starburst Galaxy NGC 253
\bibitem[Mart\'in et al.(2006)]{2006ApJS..164..450M} Mart\'in, S., Mauersberger, R., 
Mart\'in-Pintado, J., Henkel, C., and Garc\'ia-Burillo, S., ApJS,  \textbf{164}, 450-476 (2006)
%The Galactic Center as nearby extragalactic chemical laboratory
\bibitem[Mart\'in et al.(2008)]{2008Ap&SS.313..303M} Mart\'in, S., Requena-Torres, M.A., Mart\'in-Pintado, J.,  Mauersberger, R.\ 2008, ApSS,  \textbf{313}, 303-306 (2008) 
%High spatial resolution mid-infrared spectroscopy of NGC 5253: The stellar content of the embedded super-star cluster
\bibitem[Mart\'in-Hern\'andez et al.(2005)]{2005A&A...429..449M} Mart\'in-Hern\'andez, N.L., 
Schaerer, D.,  Sauvage, M., Astron. Astrophys.,  \textbf{429}, 449-467 (2005)
%The stellar content, metallicity and ionization structure of H II regions
\bibitem[Mart\'in-Hern\'andez et al.(2002)]{2002A&A...389..286M} Mart\'in-Hern\'andez, N.L., 
Vermeij, R., Tielens, A.G.G.M., van der Hulst, J.M.,  Peeters, E., Astron. Astrophys.,  
\textbf{389}, 286-294 (2002) 
\bibitem[Massey and Hunter(1998)]{1998ApJ...493..180M} Massey, P.,  Hunter, D.A., 
Astrophys.~J.,  \textbf{493}, 180 (1998)
%Dynamical constraints on star formation efficiency
\bibitem[Mathieu(1983)]{1983ApJ...267L..97M} Mathieu, R.D., Astrophys. J.,  \textbf{267}, 
L97-L101 (1983)
%Dense gas in nearby galaxies. IV - The detection of N2H(+), SiO, H(C-13)O(+), H(C-13)N, and HN(C-13)
\bibitem[Mauersberger and Henkel(1991)]{1991A&A...245..457M} Mauersberger, R.,  
Henkel, C., Astron. Astrophys.,  \textbf{245}, 457-466 (1991)
%Dense gas in nearby galaxies. XV. Hot ammonia in NGC 253, Maffei 2 and IC 342
\bibitem[Mauersberger et al.(2003)]{2003A&A...403..561M} Mauersberger, R., Henkel, C., 
Wei{\ss}, A., Peck, A.B.,  Hagiwara, Y., Astron. Astrophys.,  \textbf{403}, 561-561 (2003)
%Super Star Cluster Velocity Dispersions and Virial Masses in the M82 Nuclear Starburst
\bibitem[McCrady and Graham(2007)]{2007ApJ...663..844M} McCrady, N.,  Graham, J.R., 
Astrophys.~J.,  \textbf{663}, 844-856 (2007) 
%Kinematic Masses of Super-Star Clusters in M82 from High-Resolution Near-Infrared 
%Spectroscopy
\bibitem[McCrady et al.(2003)]{2003ApJ...596..240M} McCrady, N., Gilbert, A.M.,  
Graham, J.R., Astrophys.~J.,  \textbf{596}, 240-252 (2003)
%Mass Segregation and the Initial Mass Function of Super Star Cluster M82-F
\bibitem[McCrady et al.(2005)]{2005ApJ...621..278M} McCrady, N., Graham, J.R.,  Vacca, 
W.D., Astrophys.~J.,  \textbf{621}, 278-284 (2005)
%Theory of Star Formation
\bibitem[McKee and Ostriker(2007)]{2007ARA&A..45..565M} McKee, C.F.,  Ostriker, E.C., 
Annu. Rev. Astron. Astrophys.,  \textbf{45}, 565-687 (2007)
%Shaping the Globular Cluster Mass Function by Stellar-Dynamical Evaporation
\bibitem[McLaughlin and Fall(2008)]{2008ApJ...679.1272M} McLaughlin, D.E.,  Fall, 
S.M., Astrophys.~J.,  \textbf{679}, 1272-1287 (2008)
%Resolved Massive Star Clusters in the Milky Way and Its Satellites: Brightness Profiles 
%and a Catalog of Fundamental Parameters
\bibitem[McLaughlin and van der Marel(2005)]{2005ApJS..161..304M} McLaughlin, D.E.,  
van der Marel, R.P., ApJS,  \textbf{161}, 304-360 (2005) 
%The Fate of Star Clusters near the Galactic Center. I. Analytic Considerations
\bibitem[McMillan and Portegies Zwart(2003)]{2003ApJ...596..314M} McMillan, S.L.W.,  
Portegies Zwart, S.F., Astrophys.~J.,  \textbf{596}, 314-322 (2003)
%Molecular Gas and Star Formation in NGC 3077
\bibitem[Meier et al.(2001)]{2001AJ....122.1770M} Meier, D.S., Turner, J.L.,  Beck, S.C., 
Astron.~J.,  \textbf{122}, 1770-1781 (2001)
%Molecular Gas and the Young Starburst in NGC 5253 Revisited
\bibitem[Meier et al.(2002)]{2002AJ....124..877M} Meier, D.S., Turner, J.L.,  Beck, S.C., 
Astron.~J.,  \textbf{124}, 877-855 (2002)
%Dynamically Influenced Molecular Clouds in the Nucleus of NGC 6946: Variations in the 
%CO Isotopic Line Ratios
\bibitem[Meier and Turner(2004)]{2004AJ....127.2069M} Meier, D.S.,  Turner, J.L., Astron.~J., 
 \textbf{127}, 2069-2084 (2004)
%Spatially Resolved Chemistry in Nearby Galaxies. I. The Center of IC 342
\bibitem[Meier and Turner(2005)]{2005ApJ...618..259M} Meier, D.S.,  Turner, J.L., Astrophys.~J., 
 \textbf{618}, 259-280 (2005)
%Nuclear Bar Catalyzed Star Formation: 13CO, C18O, and Molecular Gas Properties in the Nucleus of Maffei 2
\bibitem[Meier and Turner(2008)]{MeierTurner08} Meier, D.S.,  Turner, J.L., submitted (2008)
%Nuclear Bar Catalyzed Star Formation: 13CO, C18O, and Molecular Gas Properties in the Nucleus of Maffei 2
\bibitem[Meier et al.(2008)]{2008ApJ...675..281M} Meier, D.S., Turner, J.L.,  Hurt, R.L., Astrophys.~J., 
 \textbf{675}, 281-302 (2008)
%Diagnostics of irradiated gas in galaxy nuclei. I. A far-ultraviolet and X-ray dominated region code
\bibitem[Meijerink and Spaans(2005)]{2005A&A...436..397M} Meijerink, R.,  Spaans, M., Astron. 
Astrophys.,  \textbf{436}, 397-409 (2005) 
%Irradiated ISM: Discriminating between Cosmic Rays and X-Rays
\bibitem[Meijerink et al.(2006)]{2006ApJ...650L.103M} Meijerink, R., Spaans, M.,  Israel, F.P., 
Astrophys. J.,  \textbf{650}, L103-L106 (2006) 
%The Massive Star Content of NGC 3603
\bibitem[Melena et al.(2008)]{2008AJ....135..878M} Melena, N.W., Massey, P., Morrell, N.I.,  
Zangari, A.M., Astron.~J.,  \textbf{135}, 878-891 (2008)
%Star-formation in NGC 4038/4039 from broad and narrow band photometry: 
%cluster destruction?
\bibitem[Mengel et al.(2005)]{2005A&A...443...41M} Mengel, S., Lehnert, M.D., Thatte, N.,  
Genzel, R., Astron. Astrophys.,  \textbf{443}, 41-60 (2005)
%Medium resolution 2.3 ?m spectroscopy of the massive Galactic open cluster 
%Westerlund 1
\bibitem[Mengel and Tacconi-Garman(2007)]{2007A&A...466..151M} Mengel, S.,  Tacconi-Garman, 
L.E., Astron. Astrophys.,  \textbf{466}, 151-155 (2007)
%Westerlund 1: bound or unbound?
\bibitem[Mengel and Tacconi-Garman(2008)]{2008arXiv0803.4471M} Mengel, S.,  
Tacconi-Garman, L.E., ArXiv e-prints, 803, arXiv:0803.4471 (2008)
%Starbursts and Star Clusters in the Ultraviolet
\bibitem[Meurer et al.(1995)]{1995AJ....110.2665M} Meurer, G.R., Heckman, T.M., 
Leitherer, C., Kinney, A., Robert, C.,  Garnett, D.R., Astron.~J.,  \textbf{110}, 2665-2691 (1995)
%The Properties of 30 Doradus
\bibitem[Meylan(1993)]{1993ASPC...48..588M} Meylan, G., The Globular 
Cluster-Galaxy Connection,  \textbf{48}, 588-600 (1993) 
%A radio model of the 30 Doradus region
\bibitem[Mills et al.(1978)]{1978MNRAS.185..263M} Mills, B.Y., Turtle, A.J.,  Watkinson, A., 
Mon. Not. R. Astron. Soc.,   \textbf{185}, 263-276 (1978)
\bibitem[Mirabel and Sanders(1989)]{1989ApJ...340L..53M} Mirabel, I.F.,  Sanders, D.B., 
Astrophys.~J.,  \textbf{340}, L53-56 (1989)
%The dark side of star formation in the Antennae galaxies
\bibitem[Mirabel et al.(1998)]{1998A&A...333L...1M} Mirabel, I.F., et al., Astron. Astrophys.,  
\textbf{333}, L1-L4 (1998) 
%Very Large Array Observations of the H92? Line from NGC 5253 and Henize 2-10: 
%Ionized Gas around Super Star Clusters
\bibitem[Mohan et al.(2001)]{2001ApJ...557..659M} Mohan, N.R., 
Anantharamaiah, K.R.,  Goss, W.M., Astrophys.~J.,  \textbf{557}, 659-670 (2001)
%Hubble Space Telescope Wide Field Planetary Camera 2 Observations of eta Carinae
\bibitem[Morse et al.(1998)]{1998AJ....116.2443M} Morse, J.A., Davidson, K., Bally, J., Ebbets, 
D., Balick, B.,  Frank, A., Astron.~J.,  \textbf{116}, 2443-2461 (1998)
%Dense cores in dark clouds. III - Subsonic turbulence
\bibitem[Myers(1983)]{1983ApJ...270..105M} Myers, P.C., Astrophys.~J.,  \textbf{270}, 105-118 (1983)
%The Pistol Star
\bibitem[Najarro and Figer(1998)]{1998Ap&SS.263..251N} Najarro, F.,  Figer, D.F., Ap\&SS,  
\textbf{263}, 251-254 (1998)
%Surface Brightness Profiles for a Sample of LMC, SMC, and Fornax Galaxy Globular 
%Clusters
\bibitem[Noyola and Gebhardt(2007)]{2007AJ....134..912N} Noyola, E.,  Gebhardt, K., 
Astron.~J.,  \textbf{134}, 912-925 (2007)
%The Galactic Starburst Region NGC 3603 : exciting new insights on the formation of high mass stars
\bibitem[N\"urnberger(2004)]{2004PhDT.........8N} N\"urnberger, D.E.A.\ 2004, Ph.D.Dissertation,  Univ. W{\"u}rzburg
%The molecular environment of NGC 3603. I. Spatial distribution and kinematic structure
\bibitem[N\"urnberger et al.(2002)]{2002A&A...394..253N} N\"urnberger, D.E.A., Bronfman, L., Yorke, H.W.,  Zinnecker, H., Astron. Astrophys.,  \textbf{394}, 253-269 (2002)
%Infrared observations of NGC 3603. I. New constraints on cluster radius and Ks-band 
%luminosity function
\bibitem[N\"urnberger and Petr-Gotzens(2002)]{2002A&A...382..537N} N\"urnberger, D.E.A.,  
Petr-Gotzens, M.G., Astron. Astrophys.,  \textbf{382}, 537-553 (2002)
%Hubble Space Telescope imaging of super-star clusters in NGC 1569 and NGC 1705
\bibitem[O'Connell et al.(1994)]{1994ApJ...433...65O} O'Connell, R.W., Gallagher, J.S., III, 
and Hunter, D.A., Astrophys.~J.,  \textbf{433}, 65-69 (1994)
%Hubble Space Telescope Imaging of Super Star Clusters in M82
\bibitem[O'Connell et al.(1995)]{1995ApJ...446L...1O} O'Connell, R.W., Gallagher, J.S., III, 
Hunter, D.A.,  Colley, W.N., Astrophys. J.,  \textbf{446}, L1-L4 (1995)
%Statistical Confirmation of a Stellar Upper Mass Limit
\bibitem[Oey and Clarke(2005)]{2005ApJ...620L..43O} Oey, M.S.,  Clarke, C.J., Astrophys. J., 
\textbf{620}, L43-L46 (2005)
%Molecules in galaxies
\bibitem[Omont(2007)]{2007RPPh...70.1099O} Omont, A., Reports of Progress in Physics, 
 \textbf{70}, 1099-1176 (2007)
%The Stellar Content of the Super-Star Clusters in NGC 1569
\bibitem[Origlia et al.(2001)]{2001AJ....122..815O} Origlia, L., Leitherer, C., Aloisi, A., 
Greggio, L.,  Tosi, M., Astron.~J.,  \textbf{122}, 815-824 (2001)
\bibitem[Padoan and Nordlund(2002)]{2002ApJ...576..870P} Padoan, P.,  Nordlund, {\AA}., 
Astrophys.~J.,  \textbf{576}, 870-879 (2002)
%Two Regimes of Turbulent Fragmentation and the Stellar Initial Mass Function from 
%Primordial to Present-Day Star Formation
\bibitem[Padoan et al.(2007)]{2007ApJ...661..972P} Padoan, P., Nordlund, 
{\AA}., Kritsuk, A.G., Norman, M.L.,  Li, P.S., Astrophys.~J.,  \textbf{661}, 972-981 (2007)
%Stellar Contents of the Galactic Giant H { II} Region NGC 3603
\bibitem[Pandey et al.(2000)]{2000PASJ...52..847P} Pandey, A.K., Ogura, K.,  Sekiguchi, 
K., PASJ,  \textbf{52}, 847-865 (2000)
%The origin of the Gaussian initial mass function of old globular cluster systems
\bibitem[Parmentier and Gilmore(2007)]{2007MNRAS.377..352P} Parmentier, G.,  Gilmore, 
G., Mon. Not. R. Astron. Soc.,   \textbf{377}, 352-372 (2007)
%The Shape of the Initial Cluster Mass Function: What It Tells Us about the Local Star 
%Formation Efficiency
\bibitem[Parmentier et al.(2008)]{2008ApJ...678..347P} Parmentier, G., 
Goodwin, S.P., Kroupa, P.,  Baumgardt, H., Astrophys.~J.,  \textbf{678}, 347-352 (2008)
%Polycyclic Aromatic Hydrocarbons as a Tracer of Star Formation?
\bibitem[Peeters et al.(2004)]{2004ApJ...613..986P} Peeters, E., Spoon, H.W.W.,  
Tielens, A.G.G.M., Astrophys.~J.,  \textbf{613}, 986-1003 (2004)
\bibitem[Rieke and Lebofsky(1978)]{1978ApJ...220L..37R} Rieke, G.H.,  Lebofsky, M.J., 
Astrophys. J.,  \textbf{220}, L37-L41 (1978)
%Infrared emission of extragalactic sources
\bibitem[Rieke and Lebofsky(1979)]{1979ARA&A..17..477R} Rieke, G.H.,  
Lebofsky, M.J., Annu. Rev. Astron. Astrophys.,  \textbf{17}, 477-511 (1979) 
%The nature of the nuclear sources in M82 and NGC 253
\bibitem[Rieke et al.(1980)]{1980ApJ...238...24R} Rieke, G.H., Lebofsky, 
M.J., Thompson, R.I., Low, F.J.,  Tokunaga, A.T., Astrophys.~J.,  \textbf{238}, 24-40 (1980)
%The nucleus of NGC 253
\bibitem[Rieke and Low(1975)]{1975ApJ...197...17R} Rieke, G.H.,  Low, F.J., 
Astrophys.~J.,  \textbf{197}, 17-23 
%Missing Massive Stars in Starbursts: Stellar Temperature Diagnostics and the Initial Mass Function
\bibitem[Rigby and Rieke(2004)]{2004ApJ...606..237R} Rigby, J.R.,  Rieke, G.H., 
Astrophys.~J.,  \textbf{606}, 237-257 (2004)
%VLA H53? Observations of the Central Region of the Super Star Cluster Galaxy NGC 5253
\bibitem[Rodr\'iguez-Rico et al.(2007)]{2007ApJ...670..295R} Rodr\'iguez-Rico, C.A., 
Goss, W.M., Turner, J.L., and G{\'o}mez, Y., Astrophys.~J.,  \textbf{670}, 295-300 (2007)
%Very Large Array H53? and H92? Line Observations of the Central Region of NGC 253
\bibitem[Rodr\'iguez-Rico et al.(2006)]{2006ApJ...644..914R} Rodr\'iguez-Rico, C.A., Goss, 
W.M., Zhao, J.-H., G\'omez, Y.,  Anantharamaiah, K.R., Astrophys.~J.,  \textbf{644}, 914-923 (2006)
%Detection of the H92? recombination line from the starbursts in the Circinus galaxy
% and NGC 1808
\bibitem[Roy et al.(2008)]{2008A&A...483...79R} Roy, A.L., Goss, W.M.,  Anantharamaiah, 
K.R., Astron. Astrophys.,  \textbf{483}, 79-88 (2008)
%Counterrotating Nuclear Disks in ARP 220
\bibitem[Sakamoto et al.(1999)]{1999ApJ...514...68S} Sakamoto, K., Scoville, N.Z., Yun, M.S., 
Crosas, M., Genzel, R., and Tacconi, L.J., Astrophys.~J.,  \textbf{514}, 68-76 (1999)
%CO detections and IRAS observations of bright radio spiral galaxies at CZ equal or less 
%than 9000 kilometers per second
\bibitem[Sanders and Mirabel(1985)]{1985ApJ...298L..31S} Sanders, D.B.,  Mirabel, I.F., 
Astrophys. J.,  \textbf{298}, L31-L35 (1985)
%Luminous Infrared Galaxies
\bibitem[Sanders and Mirabel(1996)]{1996ARA&A..34..749S} Sanders, D.B.,  Mirabel, I.F., 
Annu. Rev. Astron. Astrophys.,  \textbf{34}, 749-792 (1996)
\bibitem[Sanders et al.(2003)]{2003AJ....126.1607S} Sanders, D.B., Mazzarella, J.M., 
Kim, D.-C., Surace, J.A., and Soifer, B.T., Astron.~J.,  \textbf{126}, 1607-1664 (2003) 
%Giant molecular clouds in the Galaxy. II - Characteristics of discrete features
\bibitem[Sanders et al.(1985)]{1985ApJ...289..373S} 
Sanders, D.B., Scoville, N.Z.,  Solomon, P.M., Astrophys.~J.,  \textbf{289}, 373-387 (1985)
%Molecular gas in high-luminosity IRAS galaxies
\bibitem[Sanders et al.(1986)]{1986ApJ...305L..45S} Sanders, D.B., 
Scoville, N.Z., Young, J.S., Soifer, B.T., Schloerb, F.P., Rice, W.L., 
and Danielson, G.E., Astrophys. J.,  \textbf{305}, L45-L49 (1986)
%Warm ultraluminous galaxies in the IRAS survey - The transition from 
%galaxy to quasar?
\bibitem[Sanders et al.(1988)]{1988ApJ...328L..35S} Sanders, D.B., Soifer, 
B.T., Elias, J.H., Neugebauer, G.,  Matthews, K., Astrophys. J., 
 \textbf{328}, L35-L39 (1988)
%Isolated Extragalactic H II Regions
\bibitem[Sargent and Searle(1970)]{1970ApJ...162L.155S} Sargent, W.L.W.,  Searle, L., Astrophys. J., 
 \textbf{162}, L155-L160 (1970)
%A New Red Giant-based Distance Modulus of 13.3 Mpc to the 
%Antennae Galaxies and Its Consequences
\bibitem[Saviane et al.(2008)]{2008ApJ...678..179S} Saviane, I., Momany, 
Y., da Costa, G.S., Rich, R.M.,  Hibbard, J.E., Astrophys.~J.,  \textbf{678}, 179-186 (2008)
%The stellar initial mass function
\bibitem[Scalo(1986)]{1986FCPh...11....1S} Scalo, J.M., Fundamentals of Cosmic Physics, 
 \textbf{11}, 1-278 (1986)
%The IMF Revisited: A Case for Variations
\bibitem[Scalo(1998)]{1998ASPC..142..201S} Scalo, J., The Stellar 
Initial Mass Function (38th Herstmonceux Conference),  \textbf{142}, 201 (1998)
%Detection of Wolf-Rayet Stars of WN and WC Subtypes in Super--Star Clusters 
%of NGC 5253
\bibitem[Schaerer et al.(1997)]{1997ApJ...481L..75S} Schaerer, D., Contini, T., 
Kunth, D.,  Meynet, G.\ 1997, Astrophys. J., 
 \textbf{481}, L75--L78 
%Populations of WC and WN stars in Wolf-Rayet galaxies
\bibitem[Schaerer et al.(1999)]{1999A&A...341..399S} Schaerer, D., Contini, T.,  
Kunth, D., Astron. Astrophys.,  \textbf{341}, 399-417 (1999)
%New catalogue of Wolf-Rayet galaxies and high-excitation extra-galactic HII regions
\bibitem[Schaerer et al.(1999)]{1999A&AS..136...35S} Schaerer, D., Contini, T.,  Pindao, 
M., A\&AS,  \textbf{136}, 35-52 (1999)
\bibitem[Schmidt(1959)]{1959ApJ...129..243S} Schmidt, M., Astrophys.~J.,  \textbf{129}, 243-258 (1959)
%Molecular clouds and cloud cores in the inner Galaxy
\bibitem[Scoville et al.(1987)]{1987ApJS...63..821S} Scoville, N.Z., Yun, M.S., Sanders, 
D.B., Clemens, D.P., and Waller, W.H., ApJS,  \textbf{63}, 821-915 (1987)
%
\bibitem[Shepherd and Kurtz(1999)]{1999ApJ...523..690S} Shepherd, D.S.,  Kurtz, S.E., 
Astrophys.~J.,  \textbf{523}, 690-700 (1999)
%Dynamical evolution of the mass function and radial profile of the Galactic 
%globular cluster system
\bibitem[Shin et al.(2008)]{2008MNRAS.386L..67S} Shin, J., Kim, S.S.,  Takahashi, K., 
Mon. Not. R. Astron. Soc.,   \textbf{386}, L67-L71 (2008)
%Photometric properties of the Arp 220 super star clusters
\bibitem[Shioya et al.(2001)]{2001MNRAS.321...11S} Shioya, Y., Taniguchi, Y.,  
Trentham, N., Mon. Not. R. Astron. Soc.,   \textbf{321}, 11-17 (2001)
%The Pressure-confined Wind of the Massive and Compact Super Star Cluster M82-A1
\bibitem[Silich et al.(2007)]{2007ApJ...669..952S} Silich, S., Tenorio-Tagle, G.,  
Mu\~noz-Tu\~n\'on, C., Astrophys.~J.,  \textbf{669}, 952-958 (2007)
%Brackett-line observations of M82 
\bibitem[Simon et al.(1979)]{1979ApJ...227...64S} Simon, M., Simon, T.,  Joyce, R.R., 
Astrophys.~J.,  \textbf{227}, 64-66 (1979)
%The Low End of the Initial Mass Function in Young Large Magellanic Cloud Clusters. I. 
%The Case of R136
\bibitem[Sirianni et al.(2000)]{2000ApJ...533..203S} Sirianni, M., Nota, A., Leitherer, C., 
De Marchi, G.,  Clampin, M., Astrophys.~J.,  \textbf{533}, 203-214 (2000)
%Star formation rates in the Galaxy
\bibitem[Smith et al.(1978)]{1978A&A....66...65S} Smith, L.F., Mezger, P.G.,  
Biermann, P., Astron. Astrophys.,  \textbf{66}, 65-76 (1978)
%M82-F: a doomed super star cluster?
\bibitem[Smith and Gallagher(2001)]{2001MNRAS.326.1027S} Smith, L.J.,  Gallagher, J.S., 
Mon. Not. R. Astron. Soc.,   \textbf{326}, 1027-1040 (2001)
%HST/STIS optical spectroscopy of five super star clusters in the starburst galaxy M82
\bibitem[Smith et al.(2006)]{2006MNRAS.370..513S} Smith, L.J., Westmoquette, M.S., 
Gallagher, J.S., O'Connell, R.W., Rosario, D.J.,  de Grijs, R., Mon. Not. R. Astron. Soc.,  
 \textbf{370}, 513-527 (2006)
%The remarkable infrared galaxy ARP 220 = IC 4553
\bibitem[Soifer et al.(1984)]{1984ApJ...283L...1S} Soifer, B.T., et al., Astrophys. J., 
 \textbf{283}, L1-L4 (1984)
%The luminosity function and space density of the most luminous galaxies in 
%the IRAS survey
\bibitem[Soifer et al.(1986)]{1986ApJ...303L..41S} Soifer, B.T., Sanders, D.B., 
Neugebauer, G., Danielson, G.E., 
Lonsdale, C.J., Madore, B.F.,  Persson, S.E., Astrophys. J.,  \textbf{303}, L41-L44 (1986) 
%The IRAS view of the extragalactic sky
\bibitem[Soifer et al.(1987a)]{1987ARA&A..25..187S} 
Soifer, B.T., Neugebauer, G.,  Houck, 
J.R., Annu. Rev. Astron. Astrophys.,  \textbf{25}, 187-230 (1987)
%The IRAS bright galaxy sample. II - The sample and luminosity function
\bibitem[Soifer et al.(1987b)]{1987ApJ...320..238S} Soifer, B.T., Sanders, 
D.B., Madore, B.F., Neugebauer, G., Danielson, G.E., Elias, J.H., 
Lonsdale, C.J.,  Rice, W.L., Astrophys.~J.,  \textbf{320}, 238-257 (1987) 
%The Molecular Interstellar Medium in Ultraluminous Infrared Galaxies
\bibitem[Solomon et al.(1997)]{1997ApJ...478..144S} Solomon, P.M., Downes, 
D., Radford, S.J.E.,  Barrett, J.W., Astrophys.~J.,  \textbf{478}, 144-161 (1997)
%Mass, luminosity, and line width relations of Galactic molecular clouds
\bibitem[Solomon et al.(1987)]{1987ApJ...319..730S} Solomon, P.M., Rivolo, A.R., 
Barrett, J.,  Yahil, A., Astrophys.~J.,  \textbf{319}, 730-741 (1987)
%The 158 micron forbidden C II line - A measure of global star formation 
%activity in galaxies
\bibitem[Stacey et al.(1991)]{1991ApJ...373..423S} Stacey, G.J., Geis, N., 
Genzel, R., Lugten, J.B., Poglitsch, A., Sternberg, A., 
\& Townes, C.H., Astrophys. J., \textbf{373}, 423-444 (1991)
\bibitem[Stanford et al.(1990)]{1990ApJ...349..492S} Stanford, S.A., 
Sargent, A.I., Sanders, D.B.,  Scoville, N.Z., Astrophys.~J.,  \textbf{349}, 492-496 (1990)
%The Initial Mass Functions in the Super-Star Clusters NGC 1569A and NGC 1705-1
\bibitem[Sternberg(1998)]{1998ApJ...506..721S} Sternberg, A., Astrophys.~J.,  
\textbf{506}, 721-726 (1998) 
%Radio observations of super star clusters in dwarf starburst galaxies
\bibitem[Stevens et al.(2002)]{2002MNRAS.335.1079S} Stevens, I.R., Forbes, 
D.A.,  Norris, R.P., Mon. Not. R. Astron. Soc.,   \textbf{335}, 1079-1084 (2002)
%Mass functions and mass segregation in young starburst clusters
\bibitem[Stolte(2003)]{2003PhDT.........2S} Stolte, A., Ph.D.Thesis, Combined Faculties
 for the Natural Sciences and for Mathematics of the Ruperto-Carola University of Heidelberg (2003)
%The Arches Cluster: Evidence for a Truncated Mass Function?
\bibitem[Stolte et al.(2005)]{2005ApJ...628L.113S} Stolte, A., Brandner, 
W., Grebel, E.K., Lenzen, R.,  Lagrange, A.-M., Astrophys. J.,  \textbf{628}, L113-L116 (2005)
%The mass function of the Arches cluster from Gemini adaptive optics data
\bibitem[Stolte et al.(2002)]{2002A&A...394..459S} Stolte, A., Grebel, E.K., Brandner, 
W.,  Figer, D.F., Astron. Astrophys.,  \textbf{394}, 459-478 (2002)
%The Secrets of the Nearest Starburst Cluster. II. The Present-Day Mass Function in NGC 3603
\bibitem[Stolte et al.(2006)]{2006AJ....132..253S} Stolte, A., Brandner, W., Brandl, B.,  
Zinnecker, H., Astron.~J.,  \textbf{132}, 253-270 (2006)
%The radial distribution of galactic gamma rays. IV - The whole galaxy
\bibitem[Strong et al.(1988)]{1988A&A...207....1S} Strong, A.W., et al., Astron. Astrophys., 
 \textbf{207}, 1-15 (1988)
%The distribution of cosmic-ray sources in the Galaxy, ?-rays and the gradient in 
%the CO-to-H2 relation
\bibitem[Strong et al.(2004)]{2004A&A...422L..47S} Strong, A.W., Moskalenko, I.V., 
Reimer, O., Digel, S.,
 and Diehl, R., Astron. Astrophys.,  \textbf{422}, L47-L50 (2004)
%The Initial Mass Function and Stellar Content of NGC 3603
\bibitem[Sung and Bessell(2004)]{2004AJ....127.1014S} Sung, H.,  Bessell, M.S., 
Astron.~J.,  \textbf{127}, 1014-1028 (2004)
%The distribution of the interstellar medium in the Scd galaxy NGC 6946. III - Azimuthal %variations in the molecular and atomic components
\bibitem[Tacconi and Young(1990)]{1990ApJ...352..595T} Tacconi, L.J.,  Young, 
J.S., Astrophys.~J.,  \textbf{352}, 595-604 (1990)
%Equilibrium Star Cluster Formation
\bibitem[Tan et al.(2006)]{2006ApJ...641L.121T} Tan, J.C., Krumholz, M.R.,  McKee, 
C.F., Astrophys. J.,  \textbf{641}, L121-L124 (2006)
%Recent Star Formation in the Extreme Outer Disk of M83
\bibitem[Thilker et al.(2005)]{2005ApJ...619L..79T} Thilker, D.A., et al., Astrophys. J.,  
\textbf{619}, L79-L82 (2005)
%Massive Star Formation and Evolution in Starburst Galaxies: Mid-infrared Spectroscopy %with the ISO Short Wavelength Spectrometer
\bibitem[Thornley et al.(2000)]{2000ApJ...539..641T} Thornley, M.D., Schreiber, N.M.F.,
 Lutz, D., Genzel, R., Spoon, H.W.W., 
Kunze, D.,  Sternberg, A., Astrophys.~J.,  \textbf{539}, 641-657 (2000)
%The Physics and Chemistry of the Interstellar Medium
\bibitem[Tielens(2005)]{2005pcim.book.....T} Tielens, A.G.G.M., 
The Physics and Chemistry of the Interstellar Medium, by 
A.G.G.M.Tielens, pp..ISBN 0521826349.Cambridge, UK: Cambridge (2005)
University Press,  2005
%Photodissociation regions. I - Basic model. II - A model for the Orion photodissociation region
\bibitem[Tielens and Hollenbach(1985)]{1985ApJ...291..722T} Tielens, A.G.G.M.,  
Hollenbach, D., Astrophys.~J.,  \textbf{291}, 722-754 (1985)
%Photodissociation Regions - Part Two - a Model for the Orion Photodissociation Region
\bibitem[Tielens and Hollenbach(1985)]{1985ApJ...291..747T} Tielens, A.G.G.M.,  
Hollenbach, D., Astrophys.~J.,  \textbf{291}, 747-754 (1985)
%Spiral Structure of M83 - Distribution and Kinematics of the Atomic and Ionized Hydrogen
\bibitem[Tilanus and Allen(1993)]{1993A&A...274..707T} Tilanus, R.P.J.,  Allen, R.J., 
Astron. Astrophys.,  \textbf{274}, 707-729 (1993)
%Star Formation in the Field and Clusters of NGC 5253
\bibitem[Tremonti et al.(2001)]{2001ApJ...555..322T} Tremonti, C.A., Calzetti, D., 
Leitherer, C.,  Heckman, T.M., Astrophys.~J.,  \textbf{555}, 322-337 (2001) 
%Subarcsecond-Resolution Radio Maps of Nearby Spiral Galaxies
\bibitem[Tsai et al.(2006)]{2006AJ....132.2383T} Tsai, C.-W., Turner, J.L., Beck, S.C., 
Crosthwaite, 
L.P., Ho, P.T.P.,  Meier, D.S., Astron.~J.,  \textbf{132}, 2383-2397 (2006)
%The Birth of a Super-Star Cluster: NGC 5253
\bibitem[Turner and Beck(2004)]{2004ApJ...602L..85T} Turner, J.L.,  Beck, S.C., 
Astrophys. J.,  \textbf{602}, L85-L88 (2004)
%Bright radio continuum emission from star formation in the cores of nearby spiral 
%galaxies
\bibitem[Turner and Ho(1994)]{1994ApJ...421..122T} Turner, J.L.,  Ho, P.T.P., 
Astrophys. J., \textbf{421}, 122 (1994)
%An extragalactic supernebula confined by gravity
\bibitem[Turner et al.(2003)]{2003Natur.423..621T} Turner, J.L., Beck, 
S.C., Crosthwaite, L.P., Larkin, J.E., McLean, I.S.,  Meier, D.S., Nature, 
 \textbf{423}, 621-623 (2003)
%The Radio Supernebula in NGC 5253
\bibitem[Turner et al.(2000)]{2000ApJ...532L.109T} Turner, J.L., Beck, S.C.,  Ho, 
P.T.P., Astrophys. J.,  \textbf{532}, L109-L112 (2000)
%A CO Map of the Dwarf Starburst Galaxy NGC 5253
\bibitem[Turner et al.(1997)]{1997ApJ...474L..11T} Turner, J.L., Beck, S.C.,  Hurt, R.L., 
Astrophys. J.,  \textbf{474}, L11-L14 (1997)
%The Radio Properties of NGC 5253 and Its Unusual H II Regions
\bibitem[Turner et al.(1998)]{1998AJ....116.1212T} Turner, J.L., Ho, P.T.P.,  Beck, S.C., 
Astron.~J.,  \textbf{116}, 1212-1220 (1998)
%Optical spectrophotometry of Wolf-Rayet galaxies
\bibitem[Vacca and Conti(1992)]{1992ApJ...401..543V} Vacca, W.D.,  Conti, P.S., Astrophys.~J., 
 \textbf{401}, 543-558 (1992)
%Chemical Evolution of Star-Forming Regions
\bibitem[van Dishoeck and Blake(1998)]{1998ARAA..36..317V} van Dishoeck, E.F., 
 Blake, G.A., Annu. Rev. Astron. Astrophys.,  \textbf{36}, 317-368 (1998)
%Dust and super star clusters in NGC 5253
\bibitem[Vanzi and Sauvage(2004)]{2004A&A...415..509V} Vanzi, L.,  Sauvage, M., 
Astron. Astrophys.,  \textbf{415}, 509-520 (2004)
%Optimization of Starburst99 for Intermediate-Age and Old Stellar Populations
\bibitem[V\'azquez and Leitherer(2005)]{2005ApJ...621..695V} 
V\'azquez, G.A.,  Leitherer, C., Astrophys.~J.,  \textbf{621}, 695-717 (2005) 
%Characterizing the Stellar Population in NGC 1705-1
\bibitem[V\'azquez et al.(2004)]{2004ApJ...600..162V} V\'azquez, G.A., 
Leitherer, C., Heckman, T.M., Lennon, D.J., de Mello, D.F., Meurer, 
G.R.,  Martin, C.L., Astrophys.~J.,  \textbf{600}, 162-181 (2004)
%Galactic Winds
\bibitem[Veilleux et al.(2005)]{2005ARA&A..43..769V} Veilleux, S., Cecil, G.,  
Bland-Hawthorn, J., Annu. Rev. Astron. Astrophys.,  \textbf{43}, 769-826 (2005)
%A New Spectral Classification System for the Earliest O Stars: Definition of Type O2
\bibitem[Walborn et al.(2002)]{2002AJ....123.2754W} Walborn, N.R., et al.,
 Astron.~J.,  \textbf{123}, 2754-2771 (2002)
%The Discovery of Young, Luminous, Compact Stellar Clusters in the Starburst 
%Galaxy NGC 253
\bibitem[Watson et al.(1996)]{1996AJ....112..534W} Watson, A.M., et al.,
 Astron.~J.,  \textbf{112}, 534-544 (1996)
%NGC 7714 - The prototype star-burst galactic nucleus
\bibitem[Weedman et al.(1981)]{1981ApJ...248..105W} Weedman, D.W., 
Feldman, F.R., Balzano, V.A., Ramsey, L.W., 
Sramek, R.A.,  Wuu, C.-C., Astrophys.~J., \textbf{248}, 105-112 (1981)
%Evidence for a fundamental stellar upper mass limit from clustered star formation
\bibitem[Weidner and Kroupa(2004)]{2004MNRAS.348..187W} Weidner, C.,  Kroupa, P., Mon. Not. R. Astron. Soc.,   \textbf{348}, 187-191 (2004)
%R136a in the 30 Doradus nebula resolved by holographic speckle interferometry
\bibitem[Weigelt and Baier(1985)]{1985A&A...150L..18W} Weigelt, G.,  Baier, G., 
Astron. Astrophys.,  \textbf{150}, L18-L20 (1985)
%Star formation in W49A - Gravitational collapse of the molecular cloud core toward a ring of massive stars
\bibitem[Welch et al.(1987)]{1987Sci...238.1550W} Welch, W.J., Dreher, 
J.W., Jackson, J.M., Terebey, S.,  Vogel, S.N., Science,  \textbf{238}, 1550-1555 (1987)
%Hubble space telescope observations of young star clusters in NGC-4038/4039, 'the antennae' galaxies
\bibitem[Whitmore and Schweizer(1995)]{1995AJ....109..960W} Whitmore, B.C.,  
Schweizer, F., Astron.~J.,  \textbf{109}, 960-980 (1995)
%Hubble Space Telescope discovery of candidate young globular clusters in the merger %remnant NGC 7252
\bibitem[Whitmore et al.(1993)]{1993AJ....106.1354W} Whitmore, B.C., 
Schweizer, F., Leitherer, C., Borne, K.,  Robert, C., Astron.~J., 
\textbf{106}, 1354-1370 (1993)
%The Luminosity Function of Young Star Clusters in ``the Antennae'' Galaxies 
%(NGC 4038-4039)
\bibitem[Whitmore et al.(1999)]{1999AJ....118.1551W} Whitmore, B.C., 
Zhang, Q., Leitherer, C., Fall, S.M., Schweizer, F.,  Miller, B.W., Astron.~J.,  
\textbf{118}, 1551-1576 (1999)
%
\bibitem[Willner et al.(1977)]{1977ApJ...217L.121W} Willner, S.P., Soifer, 
B.T., Russell, R.W., Joyce, R.R.,  Gillett, F.C., Astrophys. J., 
 \textbf{217}, L121-L124 (1977)
%\bibitem[Wilson et al.\ 2008]{2008Ap&SS.313..297W} Wilson, C.D., et al., 
%ApSS,  \textbf{313}, 297-302 (2008) 
%High-Resolution Imaging of Molecular Gas and Dust in the Antennae (NGC 4038/39): %Super Giant Molecular Complexes
\bibitem[Wilson et al.(2000)]{2000ApJ...542..120W} Wilson, C.D., Scoville, N., Madden, S.C.,  
Charmandaris, V., Astrophys.~J.,  \textbf{542}, 120-127 (2000) 
%The Mass Function of Supergiant Molecular Complexes and Implications for Forming %Young Massive Star Clusters in the Antennae (NGC 4038/4039)
\bibitem[Wilson et al.(2003)]{2003ApJ...599.1049W} Wilson, C.D., Scoville, N., 
Madden, S.C.,  Charmandaris, V., 
Astrophys.~J.,  \textbf{599}, 1049-1066 (2003)
%CO(J = 1-0) line emission from giant molecular clouds
\bibitem[Wolfire et al.(1993)]{1993ApJ...402..195W} Wolfire, M.G., 
Hollenbach, D.,  Tielens, A.G.G.M., Astrophys.~J.,  \textbf{402}, 195-215 (1993)
%The Relationship between Gas Content and Star Formation in Molecule-rich Spiral Galaxies
\bibitem[Wong and Blitz(2002)]{2002ApJ...569..157W} Wong, T.,  Blitz, L., Astrophys.~J.,  
\textbf{569}, 157-183 (2002)
%The morphologies and physical properties of ultracompact H II regions
\bibitem[Wood and Churchwell(1989)]{1989ApJS...69..831W} Wood, D.O.S.,  
Churchwell, E.\ 1989, ApJS,  \textbf{69}, 831-895 (1989)
%The Global Rate and Efficiency of Star Formation in Spiral Galaxies as a Function of Morphology and Environment
\bibitem[Young et al.(1996)]{1996AJ....112.1903Y} Young, J.S., Allen, L., Kenney, J.D.P., 
Lesser, A.,  Rownd, B.\ 1996, Astron.~J.,  \textbf{112}, 1903-1927 (1996) 
%The molecular content of interacting and isolated galaxies The effect of environment on %the efficiency of star formation
\bibitem[Young et al.(1986)]{1986ApJ...311L..17Y} Young, J.S., Kenney, J.D., 
Tacconi, L., Claussen, M.J., Huang, 
Y.-L., Tacconi-Garman, L., Xie, S.,  Schloerb, F.P., Astrophys. J.,  \textbf{311}, L17-L21 (1986)
%Molecular gas in galaxies
\bibitem[Young and Scoville(1991)]{1991ARA&A..29..581Y} Young, J.S.,  
Scoville, N.Z., Annu. Rev. Astron. Astrophys., 
 \textbf{29}, 581-625 (1991)
%CO observations of infrared bright galaxies - The efficiency of star formation
\bibitem[Young et al.(1986)]{1986ApJ...304..443Y} Young, J.S., Schloerb, 
F.P., Kenney, J.D.,  Lord, S.D., Astrophys.~J.,  \textbf{304}, 443-458 (1986)
\bibitem[Yun et al.(1994)]
{1994Natur.372..530Y} Yun, M.S., Ho, P.T.P.,  Lo, K.Y., Nature, 
 \textbf{372}, 530-532 (1994)
%On the evolution and fate of super-massive stars
\bibitem[Yungelson et al.(2008)]{2008A&A...477..223Y} Yungelson, L.R., van den Heuvel, E.P.J., Vink, J.S., Portegies Zwart, S.F.,  de Koter, A., Astron. Astrophys.,  \textbf{477}, 223-237 (2008)
%The Mass Function of Young Star Clusters in the ``Antennae'' Galaxies
\bibitem[Zhang and Fall(1999)]{1999ApJ...527L..81Z} Zhang, Q.,  Fall, S.M., Astrophys. J.,  
\textbf{527}, L81-L84 (1999)
%Toward Understanding Massive Star Formation
\bibitem[Zinnecker and Yorke(2007)]{2007ARA&A..45..481Z} Zinnecker, H.,  
Yorke, H.W., Annu. Rev. Astron. Astrophys., 
 \textbf{45}, 481-463 (2007)
\end{thebibliography}

